High Dimensional Bayesian Optimisation and Bandits via Additive Models

Bayesian Optimisation (BO) is a technique used in optimising a $D$-dimensional function which is typically expensive to evaluate. While there have been many successes for BO in low dimensions, scaling it to high dimensions has been notoriously difficult. Existing literature on the topic are under very restrictive settings. In this paper, we identify two key challenges in this endeavour. We tackle these challenges by assuming an additive structure for the function. This setting is substantially more expressive and contains a richer class of functions than previous work. We prove that, for additive functions the regret has only linear dependence on $D$ even though the function depends on all $D$ dimensions. We also demonstrate several other statistical and computational benefits in our framework. Via synthetic examples, a scientific simulation and a face detection problem we demonstrate that our method outperforms naive BO on additive functions and on several examples where the function is not additive.

==> appExperiments.tex <==

\section{More Details on the Experiments}
\label{sec:appExperiments}


==> archive/analysisgc.tex <==

\section{Analysis}

We summarize our main theoretical contributions in Table~\ref{tb:theorySummary}.
We refer to the Basic GP UCB algorithm given in \cite{srinivas10gpbandits} by
\gpbalgo. Here, when we give rates we will ignore $\log D$ factors.
Note that our analysis suggests that \addgpbalgo has a stricty worse rate by
about a factor of $\sqrt{D/d}$ when compared to \gpbalgo even with the
\emph{simpler} additive kernel. However, this involves maximizing the
acquisition function in $D$ dimensions which is computationally very difficult.
Essentially
\addgpbalgo proposes that we ``cheat" by maximizing a UCB criterion on the
individual GPs. Even though this has a worse rate, it is much easier to maximize
the acquisition function $M$ times over $d$ dimensions. Hence, this is more
attractive in practice and is indeed confirmed by our experiments.

\begin{table}
\centering
\begin{tabular}{|l|c|c|}
\hline
Kernel & Squared Exponential & \matern \\
\hline
\rule{0pt}{3ex}
\gpbalgo on Full Kernel  & $\sqrt{ D^{D+2} T (\log T)^{D+2}}$ &
  $\sqrt{D} 2^D T^{\frac{\nu + D(D+1)}{2\nu + D(D+1)}} \log T$ \\
\hline 
\rule{0pt}{3ex}
\gpbalgo on Additive Kernel & $\sqrt{ D T d^{d+1} (\log T)^{d+2}}$ & 
  $\sqrt{Dd} 2^d T^{\frac{\nu + d(d+1)}{2\nu + d(d+1)}} \log T$ \\
\hline 
\rule{0pt}{3ex}
\addgpbalgo on Additive Kernel & $\sqrt{ D^2 T d^{d} (\log T)^{d+2}}$ & 
  $D 2^d T^{\frac{\nu + d(d+1)}{2\nu + d(d+1)}} \log T$ \\
\hline
\end{tabular}
\label{tb:theorySummary}
\caption{The Cumulative Regret for Different Algorithms}
\end{table}

\subsection{Rates on \addgpbalgo}

Our analysis in this section is similar to \cite{srinivas10gpbandits}. We will
try our best to stick to their same notation.
In the ensuing discussion, we will use $\xptt = \bigcup_j\xpttii{j}$ to denote the point
chosen by \getquerypt at the $t^{th}$ iteration. 
$\pi_t$
denotes a sequence such that $\sum_t \pi_t^{-1} = 1$. For e.g.  $\pi_t =
\pi^2 t^2/6$. 

In what follows, we will construct discretizations
$\Omegaj$ on each group $\Xcalj$ for the sake of analysis.
Let $\omega_j = |\Omegaj|$
and $\omega_m = \max_j \omega_j$.
The discretization of the individual groups induces a discretization $\Omega$
on $\Xcal$ itself, $\Omega = \{ \xpt = \bigcup_j \xptii{j} : \xptii{j} \in \Omegaj,
j = 1,\dots, M \}$. Let $\omega = |\Omega| = \prod_j \omega_j$.

We begin with some assumptions on the kernel and some Lemmas useful for us in
the proof of the main theorem. \\

\begin{definition}(Maximum Information Gain)
Let $f\sim \GP(\gpmean, \kernel)$, $y_i = f(x_i) + \epsilon$ where
$\epsilon\sim\Ncal(0, \eta^2)$. Let $A = \{x_1, \dots, x_n\}
\subset \Xcal$ be a finite subset, $\func_A$
denote the function values at these points and $y_A$
denote the noisy observations. The information between $y_A$ and
$f$ was defined in \cite{srinivas10gpbandits} to be $I(y_A; f_A)$ where
$I$ is the Shannon Mutual Information.
Further,
\cite{srinivas10gpbandits} also showed (Lemma 5.3) that
\[
I(y_A; \func_A) = \frac{1}{2} \sum_{t=1}^{n} \log(1 + \eta^{-2}
  \sigma^2_{t-1}(x_t) )
\]
where $\sigma^2_{t-1}$ is the posterior variance after observing the first $t-1$
points. The Maximum Information Gain is
$\gamma_T = \max_{A\subset \Xcal, |A| = T} I(y_A; f_A)$. $\gamma_T$ will be
useful to us in obtaining upper bounds on our algorithm. \\
\label{def:infgainGP}
\end{definition}

\begin{assumption} Each kernel $\kernelii{j}$ in the additive model satisfies
the following high probability
bound on the derivatives of the GP sample paths $\funcj$. There exists constants $a,
b >0$ such that,
\[
\PP\left( \sup_{\xii{j} \in \Xcalj} \Big|
\partialfrac{\xii{j}_i}{\funcj(\xii{j})}\Big| > L \right)
\leq a e^{-(L/b)^2}
\]
This assumption holds for stationary kernels which are four times differentiable
such as the squared exponential and \matern kernels
for $\nu > 2$ \cite{ghosal06gpconsistency, srinivas10gpbandits}. \\
\label{asm:partialDerivLipschitz}
\end{assumption}


\begin{lemma}
Pick $\delta \in (0,1)$ and set $\beta_t = 2\log(M\pi_t/\delta)$. Then
with probability $> 1-\delta$,
\[ \forall t \geq 1, \hspace{0.2in}
|f(\xptt) - \mu_{t-1}(\xptt)| \leq \betath \sumsigma{\xpttii{j}}\]
\begin{proof}
Conditioned on $\Dcal_{t-1}$, at any given $\xpt$ and $t$ we have
$f(\xptii{j}) \sim \Ncal(\gpmeanjtmo(\xptii{j}), \gpstdjtmo{j}), \; \forall j = 1,
\dots M$. Using the tail bound, $\PP(z>M) \leq e^{-M^2/2}/2$ for $z\sim
\Ncal(0,1)$ we have,
\[
\PP\left( \frac{|\funcj(\xptii{j}) -
\gpmeanjtmo(\xptii{j})|}{\gpstdjtmo(\xptii{j})} > \betath \right) \leq
e^{-\beta_t/2} = \frac{\delta}{M\pi_t}
\]
As $f(\xpt) = \sum_j\funcj(\xptii{j})$ and $\gpmeantmo(\xpt) =
\sum_j \gpmeanjtmo(\xptii{j})$ we have $|f(\xpt) - \gpmeantmo(\xpt)|
\leq \betath\sum_j \gpstdjtmo(\xptii{j})$ fixed $t$
with probability $>1-\delta/\pi_t$ .
Now using the union bound on all $t$ yields
the result. \\
\end{proof}
\label{lem:ucbptBound}
\end{lemma}

\begin{lemma}
Pick $\delta \in (0,1)$ and set $\beta_t = 2\log(\omega_m M \pi_t/\delta)$. Then
with probability $> 1-\delta$,
\[ \forall t \geq 1, \forall \xpt \in \Omega,
 \hspace{0.2in}
|f(\xpt) - \mu_{t-1}(\xpt)| \leq \betath \sumsigma{\xptii{j}}\]
\begin{proof}
As $\beta_t \geq 2\log(\omega_j M \pi_t/\delta)$ we can use a similar argument
to Lemma~\ref{lem:ucbptBound}. $\beta_t$ has an $\omega_m$ since 
we will need an additional union bound for all
elements in $\Omegaj$.
\end{proof}
\label{lem:discBound}
\end{lemma}

\begin{theorem}
Suppose $\func$ is constructed by sampling $\funcj\sim \GP(\zero, \kernelii{j})$
for $j = 1, \dots, M$ and then adding them. Further suppose all kernels
$\kernelii{j}$ satisfy assumption~\ref{asm:partialDerivLipschitz} for some
$a,b$. 
Pick $\delta\in(0,1)$ and 
% $\beta_t = 2\log(3M\pi_t/\delta) + 2d\log(Dt^2b\sqrt{3aD/\delta})$.
choose
\[
\beta_t = 2\log\left(\frac{3M\pi_t}{\delta}\right) + 
  2d\log\left(Dt^2b\sqrt{3aD/\delta}\right)
  \;\;\in \; \bigO\left( d\log t \right)
\]
for {\rm\addgpbalgo}.
Then, we obtain cumulative regret $R_T \in 
\bigOtilde\left(\sqrt{\vphantom{T^1}D\gamma_TT\log T}\right)$
where $\bigOtilde$ suppresses log dependencies on $D$. Precisely with $C_1 =
\log(1+\eta^{-2})$
\[
\PP\left( \forall T \geq 1 \;\;
R_T \leq \sqrt{8C_1\beta_TMT\gamma_t} + \pi^2/6 \right)
\geq 1 - \delta
\]

\begin{proof}
First note that by Assumption~\ref{asm:partialDerivLipschitz} and the union
bound we have,
$
\PP( \forall i\; \sup_{\xii{j} \in \Xcalj} |
{\partial \funcj(\xii{j})}/{\partial \xii{j}_i}| > L )
\leq d_i a e^{-(L/b)^2}
$.
Since, ${\partial \func(x)}/{\partial \xii{j}_i} =
{\partial \funcj(\xii{j})}/{\partial \xii{j}_i}$, we have,
\[
\PP\left( \forall i =1,\dots,D\; \sup_{x \in \Xcal} \Big|
\partialfrac{x_i}{\func(x)}\Big| > L \right)
\leq p a e^{-(L/b)^2}
\]
By setting $\delta/3=pae^{-L^2/b^2}$ we have with probability $>1-\delta/3$,
\begin{equation*}
\forall x, x' \in \Xcal, |f(x) - f(x')| \leq b \sqrt{\log(3ap/\delta)} \|x -
x'\|
\numberthis \label{eqn:fLipBound}
\end{equation*}

Now, we construct a sequence of discretizations $\Omegajt$ 
satisfying $\|\xii{j} - [\xii{j}]_t]\|_1
\leq d_j/\tau_t\;\;
\forall \xii{j} \in \Omegajt$. Here, $[\xii{j}]_t$
is the closest point to $\xii{j}$ in $\Omegajt$ in an $L_2$ sense.
A sufficient discretization is a grid with $\tau_t$
uniformly spaced points. %--i.e. .
Then it follows that for all $x\in \Omega_t$, $\|x-[x]\| \leq p/\tau_t$.
Here $\Omega_t$ is the discretization induced on $\Xcal$ by the $\Omegajt$'s
and $[x]$ is the closest point to $x$ in $\Omega_t$.
We will set $\tau_t = pt^2b\sqrt{\log(3ap/\delta)}$--therefore,
$\omega_{tj} \leq (pt^2b\sqrt{\log(3ap/\delta)})^d \defeq \omega_{mt}$.
When combining this with~\eqref{eqn:fLipBound}, we get that with probability
$>1-\delta/3$, $|\func(x) - \func([x])| \leq 1/t^2$.
% Since $\beta_t > 2\log( (pt^2b\sqrt{\log(3ap/\delta)})^d M \pi_t/ (\delta/3) )$,
By our choice of $\beta_t$
using Lemma~\ref{lem:discBound} and the union bound we have
the following 
with probability $>1-2\delta/3$ for all $t\geq 1$,
\[
|f(\xopt) - \gpmeantmo([\xopt]_t)| \leq 
|f(\xopt) - f([\xopt])| + |\func([\xopt]) - \gpmeantmo([\xopt]_t)| \leq 
\frac{1}{t^2} + \betath \sumsigma{\xoptii{j}}
\]
Further, since $\beta_t > 2\log(3M\pi_t/\delta)$ 
the result on $\xptt$ in Lemma~\ref{lem:ucbptBound} holds true
with probability $> 1- \delta/3$. Therefore with probability $>1-\delta$
\begin{align*}
r_t = \func(\xopt) - \func(\xpt) \leq \frac{1}{t^2} + \gpmeantmo(\xpt)
  + \betath\sumsigma{\xptii{j}} - f(\xpt) \leq 
  \frac{1}{t^2} + 2 \betath\sumsigma{\xptii{j}}.
\end{align*}
We can bound ${\gpstd_t(\xpt)}^2$ as follows,
\[
{\gpstd_t(\xpt)}^2= \eta^2 \eta^{-2} {\gpstd_t(\xpt)}^2
  \leq \frac{1}{\log(1+\eta^{-2})} \log\left( 1+ \eta^{-2}
{\gpstd_t(\xpt)}^2\right)
\]
The last step follows from the fact that $u^2 \leq v^2 \log(1+u^2)
/\log(1+v^2)$ for $u \leq v$ and $ {\gpstd_t(\xpt)}^2 \leq \kernel(x,x) = 1$. 
Write $C_1 = \log^{-1}(1+\eta^{-2})$.
By using Jensen's inequality and Definition~\ref{def:infgainGP},
\[
\left(\sum_{t=1}^T \sum_{j=1}^M \gpstdii{j}_{t}(\xpttii{j}) \right)^2
\leq MT\sum_{t=1}^T \sum_{j=1}^M {\gpstdii{j}_{t}(\xpttii{j})}^2
% =  MT\sum_{t=1}^T {\gpstd_t^2(\xpt)}^2 
\leq C_1 MT\sum_{t=1}^T \log\left( 1+ \eta^{-2}
{\gpstd_t(\xpt)}^2\right)
=  2 C_1 MT\gamma_T
\]
Finally we can bound the cumulative regret by,
\begin{align*}
R_T = \sum_{t=1}^T r_t \leq \frac{\pi^2}{6} + 
2\beta_T\sum_{t=1}^T \sum_{j=1}^M \gpstdii{j}_{t}(\xpttii{j}) 
\leq \frac{\pi^2}{6} + \sqrt{8C_1\beta_T M T \gamma_T}
\end{align*}
\end{proof}
\end{theorem}


\subsection{Bounding the Information Gain $\gamma_T$}

For this we will use the following theorem (Theorem 8) 
from \cite{srinivas10gpbandits}. \\

\begin{theorem}(Srinivas et al. 2010)
Suppose that $\Xcal$ is compact and $\kernel$ is a kernel on $d$ dimensions
 satisifying Assumption~\ref{asm:partialDerivLipschitz}.
Let $n_T = C_9 T^\tau \log T$ where $C_9 = 4d+2$.
For any $T_* \in \{1, \dots, \min(T, n_T)\}$,
 let $B_\kernel(T_*) = \sum_{s>T_*}
\lambda_s$. Here $(\lambda_n)_{n\in \NN}$ are the eigenvalues of $\kernel$ w.r.t
the uniform distribution over $\Xcal$. 
Then,
\begin{equation*}
\gamma_T \leq  \inf_\tau  \left(
  \frac{1/2}{1-e^{-1}} \max_{r\in\cbr{1,\dots,T}} \left( T_* \log(r n_T/
\eta^2) + C_9 \eta^2 (1 - r/T) (T^{\tau+1} B_\kernel(T_*) + 1) \log T \right)
  + \bigO(T^{1-\tau /d}) 
\right)
\end{equation*}
\label{thm:srinivas}
\end{theorem}

\subsubsection{Additive Squared Exponential Kernels}

\begin{theorem}(Information Gain for Additive Squared Exponential Kernel) Consider a kernel
of the form,
\[
\kernel(x,x') = \kernelii{1}(\xii{1}, \xiip{1}) + \dots +
  \kernelii{M}(\xii{M}, \xiip{M})
\]
where $\kernelii{i}$ is a $d_i$ dimensional squared exponential kernel.
As before we will assume $d_i \leq d\; \forall i$. For this kernel, $\gamma_T
\in \bigO\left(Dd^d (\log T)^{d+1}\right)$.

\begin{proof}
\emph{ Our proof uses ideas from \cite{srinivas10gpbandits,
seeger08information}.}

We will use some bounds on the eigenvalues for the simple squared exponential
kernel given in \cite{seeger08information}. It was shown that the eigenvalues
$\{\lambdaii{i}_s\}$ of $\kernelii{i}$ satisfied $\lambdaii{i}_s \leq
c^dB^{s^{1/d_i}}$ where $B < 1$ (See Remark~\ref{rmk:eigvaldistros}).
Since the kernel is additive, and $\xii{i} \cap
\xii{j} = \emptyset$ the eigenfunctions corresponding to $\kernelii{i}$ and
$\kernelii{j}$ will be orthogonal. Hence the eigenvalues of $\kernel$ will
just be the union of the eigenvalues of the individual kernels -- i.e. 
$\{\lambda_s\} = \bigcup_{j=1}^M \{\lambdaii{j}_s \}$.  
As $B<1$, $\lambdaii{i}_s \leq c^dB^{s^{1/d}}$. Let $\Thash = \floor{T_*/M}$ and
$\alpha = -\log B$.
Then,
\begin{align*}
B_\kernel(T_*) &= \sum_{s>T_*} \lambda_s \leq Mc \sum_{s>\Thash} B^{s^{1/d}} \\
  &\leq c^dM \left( B^{\Thash^{1/d}} + \int_{\Thash}^\infty \exp(-\alpha x ^{1/d})
            \right) \ud x \\
  &\leq c^dM \left( B^{\Thash^{1/d}} + d \alpha^{-d} \Gamma(d, \alpha \Thash^{1/d})
            \right) \\ 
  &\leq c^dMe^{-\alpha \Thash^{1/d}} 
  \left( 1 + d! d \alpha^{-d} (\alpha \Thash^{1/d})^{d-1} \right)
\end{align*}
The last step holds true whenever $\alpha \Thash^{1/d} \geq 1$.
Here in the second step we bound the series by an integral used in the Maclaurin
Cauchy Integral test. In the second step we used the substitution $y =
\alpha x^{1/d}$ to simplify the integral. Here $\Gamma(s,x) = \int_x^\infty
t^{s-1} e^{-t} \ud t$ is the (upper) incomplete Gamma function. In the last step
we have used the following identity and the bound for integral $s$ and $x\geq 1$
\[
\Gamma(s,x) = (s-1)! e^{-x} \sum_{k=0}^{s-1} \frac{x^k}{k!} \leq s! e^{-x} x^{d-1}
\]
By using $\tau = d$ and by using
$T_* \leq (M+1) \Thash$, we
use Theorem~\ref{thm:srinivas} to obtain the following bound on $\gamma_T$,
\begin{align*}
\gamma_T &\leq 
  \frac{1/2}{1-e^{-1}} \max_{r\in\cbr{1,\dots,T}} \bigg( (M+1) \Thash \log(r n_T/
\eta^2) + \\
 &\hspace{0.2in} 
  C_9 \eta^2 (1 - r/T)  \log T \left( 1 + c^dMe^{-\alpha \Thash^{1/d}} T^{d+1} 
  \left( 1 + d! d \alpha^{-d} (\alpha \Thash^{1/d})^{d-1} \right)
  \right) \bigg)
\label{eqn:gammarbound} \numberthis
\end{align*}
Now we need to pick $\Thash$ so as to balance these two terms. We will choose
$\Thash = \left(\frac{\log(Tn_T)}{\alpha}\right)^d $ which is less than $\min(T,
n_T)/M$ for sufficiently large $T$. 
Then $e^{-\alpha \Thash^{1/d}} = 1/Tn_T$. Then the first term $S_1$ inside the
paranthesis is,
\begin{align*}
S_1 = (M+1) \log^d\left(\frac{Tn_T}{\alpha}\right)
        \log\left(\frac{rn_T}{\eta^2}\right) 
  &\in \bigO\left(M \left(\log(Tn_T)\right)^{d}\log(rn_T) \right) \\
  &\in \bigO\left(M \left(\log(T^{d+1}\log T)\right)^{d} \log(rT^d \log T)\right) \\
  &\in \bigO\left(M d^{d+1} (\log T)^{d+1} + M d^d (\log T)^d\log(r) \right)
\end{align*}
Note that the constant in front has exponential dependence on $d$ but we ignore
it since we already have $d^d$, $(\log T)^d$ terms.
The second term $S_2$ becomes,
\begin{align*}
S_2 &= 
  C_9 \eta^2 (1 - r/T)  \log T \left( 1 + \frac{c^dM}{Tn_T} T^{d+1} 
  \left( 1 + d! d \alpha^{-d} (\log(Tn_T)^{d-1} \right) 
  \right) \bigg) \\
  &\leq C_9 \eta^2 (1 - r/T)  \left( \log T  + \frac{c^dM}{C_9}  
  \left( 1 + d! d \alpha^{-d} (\log(Tn_T)^{d-1} \right) 
  \right) \bigg) \\
  &\leq C_9 \eta^2 (1 - r/T)  \left( \bigO(\log T) + \bigO(1) +
   \bigO(d! d^{d} (\log T)^{d-1}) \right) \bigg) \\
  &\in \bigO\left( (1-r/T)d! d^{d} (\log T)^{d-1} \right)
\end{align*}
Since $S_1$ dominates $S_2$, we should choose $r=T$ to maximize the RHS
in~\eqref{eqn:gammarbound}. This gives us,
\[
\gamma_T 
\;\in\; \bigO\left(M d^{d+1} (\log T)^{d+1}\right) 
\;\in\; \bigO\left(D d^{d} (\log T)^{d+1} \right) 
\]
\end{proof}
\end{theorem}


\subsubsection{Additive \matern Kernels}

\begin{theorem}(Information Gain for \matern Kernel) 
Consider a kernel
of the form,
\[
\kernel(x,x') = \kernelii{1}(\xii{1}, \xiip{1}) + \dots +
  \kernelii{M}(\xii{M}, \xiip{M})
\]
where $\kernelii{i}$ is a $d_i$ dimensional \matern kernel with parameter $\nu
> 2$.
As before we will assume $d_i \leq d\; \forall i$. For this kernel, $\gamma_T
\in \bigO\left(M 2^d T^{\frac{d(d+1)}{2\nu + d(d+1)}} \log(MT) \right)$.

\begin{proof}
Once again, we use bounds given in \cite{seeger08information}. 
It was shown that the eigenvalues $\{\lambdaii{i}_s\}$ for $\kernelii{i}$
satisfied $\lambdaii{i}_s \leq c^ds^{-\frac{2\nu+d_j}{d_j}}$
(See Remark~\ref{rmk:eigvaldistros}). By following a
similar argument to above we have 
$\{\lambda_s\} = \bigcup_{j=1}^M \{\lambdaii{j}_s \}$ and
$\lambdaii{i}_s \leq c^ds^{-\frac{2\nu+d}{d}}$. Let $\Thash = \floor{T_*/M}$.
Then,
\begin{align*}
B_\kernel(T_*) = \sum_{s>T_*} \lambda_s 
  \leq Mc^d\sum_{s>\Thash} s^{-\frac{2\nu+d}{d}} 
  \leq Mc^d\left( \Thash^{-\frac{2\nu+d}{d}} + 
      \int_{\Thash}^\infty s^{-\frac{2\nu+d}{d}}\right) 
  \leq C_8 2^d M\Thash^{1-\frac{2\nu+d}{d}}
%   \in \bigO\left(M\Thash^{1-\frac{2\nu+d}{d}} \right)
\end{align*}
where $C_8$ is an appropriate constant.
We set $\Thash = (Tn_T)^{\frac{d}{2\nu+d}} (\log(Tn_T))^{-\frac{d}{2\nu+d}}$ and
accordingly we have the following bound on $\gamma_T$ as a function of $\Thash \in
\{1,\dots, \min(T, n_T)/M\}$,
\begin{align*}
\gamma_T \leq 
  \inf_\tau \Bigg(
  \frac{1/2}{1-e^{-1}} \max_{r\in\cbr{1,\dots,T}} \bigg( (M+1) \Thash \log(r n_T/
\eta^2) +  
  C_9 \eta^2 (1 - r/T)   \left( \log T + C_8 2^d M \Thash \log(Tn_T) \right)
  \bigg) + \bigO(T^{1-\tau/d}) \Bigg)
\label{eqn:gammarboundmatern} \numberthis
\end{align*}
Since this is a concave function on $r$ we can find the optimum by setting the
derivative w.r.t $r$ to be zero. We get $r \in \bigO(T/2^d\log(Tn_T))$ and hence,
\begin{align*}
\gamma_T &\in \inf_\tau 
\left( \bigO\left( M \Thash \log\left(\frac{Tn_T}{2^d\log(Tn_T)}\right) \right)
  + \bigO\left(M 2^d \Thash \log(Tn_T) \right)
      + \bigO(T^{1-\tau/d}) \right) \\
&\in \inf_\tau \left(\bigO \left(M 2^d \log(Tn_T)
   \left(\frac{T^{\tau+1}\log(T)}{(\tau+1)\log(T) + \log\log T}\right)^\frac{d}{2\nu+d}
   \right) 
  + \bigO(T^{1-\tau/d}) \right) \\
&\in \inf_\tau \left(\bigO \left(M2^d\log(Tn_T)
   T^{\frac{(\tau+1)d}{2\nu+d}} \right) 
  + \bigO(T^{1-\tau/d}) \right) \\
&\in \bigO\left( M 2^d T^{\frac{d(d+1)}{2\nu + d(d+1)}} \log(T) \right)
\end{align*}
Here in the second step we have substitued the values for $\Thash$ first and
then $n_T$. In the last step we have balanced the polynomial dependence on $T$
in both terms by setting $\tau = \frac{2\nu d}{2\nu + d(d+1)}$. \\
\end{proof}
\label{thm:infGainMatern}
\end{theorem}

\begin{remark}
The eigenvalues and eigenfunctions for the kernel are defined with respect to a
base distribution on $\Xcal$. In the development of Theorem~\ref{thm:srinivas},
\cite{srinivas10gpbandits} draw $n_T$ samples from the uniform distribution on
$\Xcal$. Hence, the eigenvalues/eigenfunctions should be w.r.t the uniform
distribution. The bounds given in \cite{seeger08information} are for the uniform
distribution for the \matern kernel and a Gaussian Distribution for the Squared
Exponential Kernel. For the latter case, \cite{srinivas10gpbandits} argue that
the uniform distribution still satisfies the required tail constraints and
therefore the bounds would only differ up to constants.
\label{rmk:eigvaldistros}
\end{remark}


==> archive/appRates.tex <==

\subsection{Rates on \addgpbalgo}
\label{sec:appAnalysisRates}

Our analysis in this section is similar to \cite{srinivas10gpbandits}. We will
try our best to stick to their same notation.
In the ensuing discussion, we will use $\xptt = \bigcup_j\xpttii{j}$ to denote the point
chosen by \gpbalgo at the $t^{th}$ iteration. 
$\pi_t$
denotes a sequence such that $\sum_t \pi_t^{-1} = 1$. For e.g. when we use
$\pi_t = \pi^2 t^2/6$ below, we obtain the rates in Theorem~\ref{thm:addGPBthm}.
Denote $p = \sum_j d_j$.

In what follows, we will construct discretisations
$\Omegaj$ on each group $\Xcalj$ for the sake of analysis.
Let $\omega_j = |\Omegaj|$
and $\omega_m = \max_j \omega_j$.
The discretisation of the individual groups induces a discretisation $\Omega$
on $\Xcal$ itself, $\Omega = \{ \xpt = \bigcup_j \xptii{j} : \xptii{j} \in \Omegaj,
j = 1,\dots, M \}$. Let $\omega = |\Omega| = \prod_j \omega_j$.
We first establish the following two lemmas before we prove
Theorem~\ref{thm:addGPBthm}.
\\[\thmparaspacing]

\begin{lemma}
Pick $\delta \in (0,1)$ and set $\beta_t = 2\log(M\pi_t/\delta)$. Then
with probability $> 1-\delta$,
\[ \forall t \geq 1, \hspace{0.2in}
|f(\xptt) - \mu_{t-1}(\xptt)| \leq \betath \sumsigma{\xpttii{j}}\]
\begin{proof}
Conditioned on $\Dcal_{t-1}$, at any given $\xpt$ and $t$ we have
$f(\xptii{j}) \sim \Ncal(\gpmeanjtmo(\xptii{j}), \gpstdjtmo{j}), \; \forall j = 1,
\dots M$. Using the tail bound, $\PP(z>M) \leq \frac{1}{2}e^{-M^2/2}$ for $z\sim
\Ncal(0,1)$ we have,
\[
\PP\left( \frac{|\funcj(\xptii{j}) -
\gpmeanjtmo(\xptii{j})|}{\gpstdjtmo(\xptii{j})} > \betath \right) \leq
e^{-\beta_t/2} = \frac{\delta}{M\pi_t}
\]
As $f(\xpt) = \sum_j\funcj(\xptii{j})$ and $\gpmeantmo(\xpt) =
\sum_j \gpmeanjtmo(\xptii{j})$ we have $|f(\xpt) - \gpmeantmo(\xpt)|
\leq \betath\sum_j \gpstdjtmo(\xptii{j})$ fixed $t$
with probability $>1-\delta/\pi_t$ .
Now using the union bound on all $t$ yields
the result. \\[\thmparaspacing]
\end{proof}
\label{lem:ucbptBound}
\end{lemma}

\begin{lemma}
Pick $\delta \in (0,1)$ and set $\beta_t = 2\log(\omega_m M \pi_t/\delta)$. Then
with probability $> 1-\delta$,
\[ \forall t \geq 1, \forall \xpt \in \Omega,
 \hspace{0.2in}
|f(\xpt) - \mu_{t-1}(\xpt)| \leq \betath \sumsigma{\xptii{j}}\]
\begin{proof}
As $\beta_t \geq 2\log(\omega_j M \pi_t/\delta)$ we can use a similar argument
to Lemma~\ref{lem:ucbptBound}. $\beta_t$ has an $\omega_m$ since 
we will need an additional union bound for all
elements in $\Omegaj$. \\[\thmparaspacing]
\end{proof}
\label{lem:discBound}
\end{lemma}


\subsubsection{\textbf{Proof of Theorem~\ref{thm:addGPBthm}}}
\begin{proof}
First note that by Assumption~\ref{asm:partialDerivLipschitz} and the union
bound we have,
$
\PP( \forall i\; \sup_{\xii{j} \in \Xcalj} |
{\partial \funcj(\xii{j})}/{\partial \xii{j}_i}| > L )
\leq d_i a e^{-(L/b)^2}
$.
Since, ${\partial \func(x)}/{\partial \xii{j}_i} =
{\partial \funcj(\xii{j})}/{\partial \xii{j}_i}$, we have,
\[
\PP\left( \forall i =1,\dots,D\; \sup_{x \in \Xcal} \Big|
\partialfrac{x_i}{\func(x)}\Big| > L \right)
\leq p a e^{-(L/b)^2}
\]
By setting $\delta/3=pae^{-L^2/b^2}$ we have with probability $>1-\delta/3$,
\begin{equation*}
\forall x, x' \in \Xcal, |f(x) - f(x')| \leq b \sqrt{\log(3ap/\delta)} \|x -
x'\|
\numberthis \label{eqn:fLipBound}
\end{equation*}

Now, we construct a sequence of discretisations $\Omegajt$ 
satisfying $\|\xii{j} - [\xii{j}]_t]\|_1
\leq d_j/\tau_t\;\;
\forall \xii{j} \in \Omegajt$. Here, $[\xii{j}]_t$
is the closest point to $\xii{j}$ in $\Omegajt$ in an $L_2$ sense.
A sufficient discretisation is a grid with $\tau_t$
uniformly spaced points. %--i.e. .
Then it follows that for all $x\in \Omega_t$, $\|x-[x]\| \leq p/\tau_t$.
Here $\Omega_t$ is the discretisation induced on $\Xcal$ by the $\Omegajt$'s
and $[x]$ is the closest point to $x$ in $\Omega_t$.
We will set $\tau_t = pt^2b\sqrt{\log(3ap/\delta)}$--therefore,
$\omega_{tj} \leq (pt^2b\sqrt{\log(3ap/\delta)})^d \defeq \omega_{mt}$.
When combining this with~\eqref{eqn:fLipBound}, we get that with probability
$>1-\delta/3$, $|\func(x) - \func([x])| \leq 1/t^2$.
% Since $\beta_t > 2\log( (pt^2b\sqrt{\log(3ap/\delta)})^d M \pi_t/ (\delta/3) )$,
By our choice of $\beta_t$
using Lemma~\ref{lem:discBound} and the union bound we have
the following 
with probability $>1-2\delta/3$ for all $t\geq 1$,
\[
|f(\xopt) - \gpmeantmo([\xopt]_t)| \leq 
|f(\xopt) - f([\xopt])| + |\func([\xopt]) - \gpmeantmo([\xopt]_t)| \leq 
\frac{1}{t^2} + \betath \sumsigma{\xoptii{j}}
\]
Further, since $\beta_t > 2\log(3M\pi_t/\delta)$ 
the result on $\xptt$ in Lemma~\ref{lem:ucbptBound} holds true
with probability $> 1- \delta/3$. Therefore with probability $>1-\delta$
\begin{align*}
r_t = \func(\xopt) - \func(\xpt) \leq \frac{1}{t^2} + \gpmeantmo(\xpt)
  + \betath\sumsigma{\xptii{j}} - f(\xpt) \leq 
  \frac{1}{t^2} + 2 \betath\sumsigma{\xptii{j}}.
\end{align*}
We can bound ${\gpstd_t(\xpt)}^2$ as follows,
\[
{\gpstd_t(\xpt)}^2= \eta^2 \eta^{-2} {\gpstd_t(\xpt)}^2
  \leq \frac{1}{\log(1+\eta^{-2})} \log\left( 1+ \eta^{-2}
{\gpstd_t(\xpt)}^2\right)
\]
The last step follows from the fact that $u^2 \leq v^2 \log(1+u^2)
/\log(1+v^2)$ for $u \leq v$ and $ {\gpstd_t(\xpt)}^2 \leq \kernel(x,x) = 1$. 
Write $C_1 = \log^{-1}(1+\eta^{-2})$.
By using Jensen's inequality and Definition~\ref{def:infgainGP},
\[
\left(\sum_{t=1}^T \sum_{j=1}^M \gpstdii{j}_{t}(\xpttii{j}) \right)^2
\leq MT\sum_{t=1}^T \sum_{j=1}^M {\gpstdii{j}_{t}(\xpttii{j})}^2
% =  MT\sum_{t=1}^T {\gpstd_t^2(\xpt)}^2 
\leq C_1 MT\sum_{t=1}^T \log\left( 1+ \eta^{-2}
{\gpstd_t(\xpt)}^2\right)
=  2 C_1 MT\gamma_T
\]
Finally we can bound the cumulative regret by,
\begin{align*}
R_T = \sum_{t=1}^T r_t \leq \frac{\pi^2}{6} + 
2\beta_T\sum_{t=1}^T \sum_{j=1}^M \gpstdii{j}_{t}(\xpttii{j}) 
\leq \frac{\pi^2}{6} + \sqrt{8C_1\beta_T M T \gamma_T}
\end{align*}
\end{proof}


==> archive/gc.tex <==


% We will denote the groups via super scripts and the
% % individual dimensions via subscripts. Therefore, $\xii{j}$ refers to the
% % $j$\superscript{th}
% % group, $x_i$ refers to the $i$\superscript{th} 
% % dimension and $\xii{j}_i$ refers to the $j$\superscript{th} 
% % dimension in the $i$\superscript{th} group. 
% We will used paranthesized superscripts to index the groups.
% Boldfaced font 
% indicates the points chosen by the algorithm for querying.
% $\xptt$ indicates the $t^{th}$ query point and
% $\xpttii{j}$, $\xpt_{ti}$, $\xptii{j}_{ti}$ refer respectively to the 
% $j$\superscript{th} group,
% the $i$\superscript{th} dimension and the $j$\superscript{th}
%  dimension of the $i$\superscript{th} group of the $t^{th}$
% query point.
% $\xvect, \yvect$ will denote $\{\xpt_1, \dots, \xpt_t\}$ and
% $\{\ypt_1, \dots, \ypt_t\}$. Denote all input output pairs up to time $t$ by
% $(\xvect, \yvect)$ by $\Dcal_t$.
% Denote the true function values up to time $t$ by $\funcvect = \{\func(\xpt_1),
% \dots, \func(\xpt_t)\}$.
% Denote the \emph{unique}
% optimum point of the function by $\xopt = \bigcup_j \xoptii{j}$.
% For this analysis we will assume w.l.o.g that $\kernel(x,x) = 1$.

% \begin{algorithm}
% \textbf{Input: } Decomposition $\Xcal =\bigcup_{j=1}^M \Xcalii{j} $,
% GP Posterior Means and Variances $\gpmeanii{j}, \gpstdii{j} $ for
% $j=1,\dots, M$.\\
% \textbf{Output: } Next query point $\xpt$
% % For $t = 1,2 \dots$
% \begin{enumerate}
% \item \textbf{for} $j=1,\dots,M$, \hspace{0.11in}
%   $\xptii{j} \leftarrow \argmax_{z\in \Xcalii{j}} \gpmeanii{j}(z) + 
%   \sqrt{\beta_t} \gpstdii{j}(z)$ 
% \item  Return $\xpt\leftarrow \bigcup_{j=1}^M \xptii{j}$. %Query $\func$ at $\xptt$.
% \end{enumerate}
% \caption{\getqueryptarg{(\Xcalii{j})_{j=1}^M}
%   {(\gpmeanii{j}, \gpstdii{j})_{j=1}^M}
%   \label{alg:getquerypt} }
% \end{algorithm}


==> archive/old-intro.tex <==

\section{Introduction}
% \label{sec:intro}

intro-GP bandits

intro - BO

introduce acquisition function $\utilt$,

We assume that we will observe the function with some additive white Gaussian
noise with variance $\eta^2 > 0$ when we query at $x$. Precisely,
\begin{equation}
y = f(x) + \eta \epsilon
\end{equation}
where $\epsilon\sim \Ncal(0,1)$.


Both GPB and BO first estimates the posterior Gaussian Process using the $(x,y)$
pairs queried thus far. Then we construct an acquisition function using the
points developed th




\toworkon{Choosing a simpler kernel is advantageous even if the function is not
additive for multiple reasons. When
we can afford only a few queries ?}

If we run \gpbalgo of \cite{srinivas10gpbandits} we get improved regret since
the additive structure essentially assumes a simpler kernel. Hence, this addresses our
statistical concern. But it still requires maximizing an acquisition function in
$D$ dimensions. This is undesirable as it requires exponential in $D$ effort.
To address this concern, we propose 
constructing a UCB acquisition function for each of the individual GPs and
maximizing them individually. This only requires linear in $D$ and
exponential in $d$ effort.



There are two main components to the algorithm we propose. The first involves
inference on the individual GPs in the additive model in~\eqref{eqn:addmodel}.
The latter is on maximizing a UCB acquisition function on each of these GPs.


==> archive/oldAppAnalysis.tex <==

\section{Analysis}
\label{sec:analysis}

\subsection{Rates on \addgpbalgo}
\label{sec:appAnalysisRates}

Our analysis in this section is similar to \cite{srinivas10gpbandits}. We will
try our best to stick to their same notation.
In the ensuing discussion, we will use $\xptt = \bigcup_j\xpttii{j}$ to denote the point
chosen by \gpbalgo at the $t^{th}$ iteration. 
$\pi_t$
denotes a sequence such that $\sum_t \pi_t^{-1} = 1$. For e.g. when we use
$\pi_t = \pi^2 t^2/6$ below, we obtain the rates in~\ref{thm:addGPBthm}.
Denote $p = \sum_j d_j$.

In what follows, we will construct discretizations
$\Omegaj$ on each group $\Xcalj$ for the sake of analysis.
Let $\omega_j = |\Omegaj|$
and $\omega_m = \max_j \omega_j$.
The discretization of the individual groups induces a discretization $\Omega$
on $\Xcal$ itself, $\Omega = \{ \xpt = \bigcup_j \xptii{j} : \xptii{j} \in \Omegaj,
j = 1,\dots, M \}$. Let $\omega = |\Omega| = \prod_j \omega_j$.
We first establish the following two lemmas before we prove
Theorem~\ref{thm:addGPBthm}.
\\[\thmparaspacing]

\begin{lemma}
Pick $\delta \in (0,1)$ and set $\beta_t = 2\log(M\pi_t/\delta)$. Then
with probability $> 1-\delta$,
\[ \forall t \geq 1, \hspace{0.2in}
|f(\xptt) - \mu_{t-1}(\xptt)| \leq \betath \sumsigma{\xpttii{j}}\]
\begin{proof}
Conditioned on $\Dcal_{t-1}$, at any given $\xpt$ and $t$ we have
$f(\xptii{j}) \sim \Ncal(\gpmeanjtmo(\xptii{j}), \gpstdjtmo{j}), \; \forall j = 1,
\dots M$. Using the tail bound, $\PP(z>M) \leq \frac{1}{2}e^{-M^2/2}$ for $z\sim
\Ncal(0,1)$ we have,
\[
\PP\left( \frac{|\funcj(\xptii{j}) -
\gpmeanjtmo(\xptii{j})|}{\gpstdjtmo(\xptii{j})} > \betath \right) \leq
e^{-\beta_t/2} = \frac{\delta}{M\pi_t}
\]
As $f(\xpt) = \sum_j\funcj(\xptii{j})$ and $\gpmeantmo(\xpt) =
\sum_j \gpmeanjtmo(\xptii{j})$ we have $|f(\xpt) - \gpmeantmo(\xpt)|
\leq \betath\sum_j \gpstdjtmo(\xptii{j})$ fixed $t$
with probability $>1-\delta/\pi_t$ .
Now using the union bound on all $t$ yields
the result. \\[\thmparaspacing]
\end{proof}
\label{lem:ucbptBound}
\end{lemma}

\begin{lemma}
Pick $\delta \in (0,1)$ and set $\beta_t = 2\log(\omega_m M \pi_t/\delta)$. Then
with probability $> 1-\delta$,
\[ \forall t \geq 1, \forall \xpt \in \Omega,
 \hspace{0.2in}
|f(\xpt) - \mu_{t-1}(\xpt)| \leq \betath \sumsigma{\xptii{j}}\]
\begin{proof}
As $\beta_t \geq 2\log(\omega_j M \pi_t/\delta)$ we can use a similar argument
to Lemma~\ref{lem:ucbptBound}. $\beta_t$ has an $\omega_m$ since 
we will need an additional union bound for all
elements in $\Omegaj$. \\[\thmparaspacing]
\end{proof}
\label{lem:discBound}
\end{lemma}


\subsubsection{\textbf{Proof of Theorem~\ref{thm:addGPBthm}}}
\begin{proof}
First note that by Assumption~\ref{asm:partialDerivLipschitz} and the union
bound we have,
$
\PP( \forall i\; \sup_{\xii{j} \in \Xcalj} |
{\partial \funcj(\xii{j})}/{\partial \xii{j}_i}| > L )
\leq d_i a e^{-(L/b)^2}
$.
Since, ${\partial \func(x)}/{\partial \xii{j}_i} =
{\partial \funcj(\xii{j})}/{\partial \xii{j}_i}$, we have,
\[
\PP\left( \forall i =1,\dots,D\; \sup_{x \in \Xcal} \Big|
\partialfrac{x_i}{\func(x)}\Big| > L \right)
\leq p a e^{-(L/b)^2}
\]
By setting $\delta/3=pae^{-L^2/b^2}$ we have with probability $>1-\delta/3$,
\begin{equation*}
\forall x, x' \in \Xcal, |f(x) - f(x')| \leq b \sqrt{\log(3ap/\delta)} \|x -
x'\|
\numberthis \label{eqn:fLipBound}
\end{equation*}

Now, we construct a sequence of discretizations $\Omegajt$ 
satisfying $\|\xii{j} - [\xii{j}]_t]\|_1
\leq d_j/\tau_t\;\;
\forall \xii{j} \in \Omegajt$. Here, $[\xii{j}]_t$
is the closest point to $\xii{j}$ in $\Omegajt$ in an $L_2$ sense.
A sufficient discretization is a grid with $\tau_t$
uniformly spaced points. %--i.e. .
Then it follows that for all $x\in \Omega_t$, $\|x-[x]\| \leq p/\tau_t$.
Here $\Omega_t$ is the discretization induced on $\Xcal$ by the $\Omegajt$'s
and $[x]$ is the closest point to $x$ in $\Omega_t$.
We will set $\tau_t = pt^2b\sqrt{\log(3ap/\delta)}$--therefore,
$\omega_{tj} \leq (pt^2b\sqrt{\log(3ap/\delta)})^d \defeq \omega_{mt}$.
When combining this with~\eqref{eqn:fLipBound}, we get that with probability
$>1-\delta/3$, $|\func(x) - \func([x])| \leq 1/t^2$.
% Since $\beta_t > 2\log( (pt^2b\sqrt{\log(3ap/\delta)})^d M \pi_t/ (\delta/3) )$,
By our choice of $\beta_t$
using Lemma~\ref{lem:discBound} and the union bound we have
the following 
with probability $>1-2\delta/3$ for all $t\geq 1$,
\[
|f(\xopt) - \gpmeantmo([\xopt]_t)| \leq 
|f(\xopt) - f([\xopt])| + |\func([\xopt]) - \gpmeantmo([\xopt]_t)| \leq 
\frac{1}{t^2} + \betath \sumsigma{\xoptii{j}}
\]
Further, since $\beta_t > 2\log(3M\pi_t/\delta)$ 
the result on $\xptt$ in Lemma~\ref{lem:ucbptBound} holds true
with probability $> 1- \delta/3$. Therefore with probability $>1-\delta$
\begin{align*}
r_t = \func(\xopt) - \func(\xpt) \leq \frac{1}{t^2} + \gpmeantmo(\xpt)
  + \betath\sumsigma{\xptii{j}} - f(\xpt) \leq 
  \frac{1}{t^2} + 2 \betath\sumsigma{\xptii{j}}.
\end{align*}
We can bound ${\gpstd_t(\xpt)}^2$ as follows,
\[
{\gpstd_t(\xpt)}^2= \eta^2 \eta^{-2} {\gpstd_t(\xpt)}^2
  \leq \frac{1}{\log(1+\eta^{-2})} \log\left( 1+ \eta^{-2}
{\gpstd_t(\xpt)}^2\right)
\]
The last step follows from the fact that $u^2 \leq v^2 \log(1+u^2)
/\log(1+v^2)$ for $u \leq v$ and $ {\gpstd_t(\xpt)}^2 \leq \kernel(x,x) = 1$. 
Write $C_1 = \log^{-1}(1+\eta^{-2})$.
By using Jensen's inequality and Definition~\ref{def:infgainGP},
\[
\left(\sum_{t=1}^T \sum_{j=1}^M \gpstdii{j}_{t}(\xpttii{j}) \right)^2
\leq MT\sum_{t=1}^T \sum_{j=1}^M {\gpstdii{j}_{t}(\xpttii{j})}^2
% =  MT\sum_{t=1}^T {\gpstd_t^2(\xpt)}^2 
\leq C_1 MT\sum_{t=1}^T \log\left( 1+ \eta^{-2}
{\gpstd_t(\xpt)}^2\right)
=  2 C_1 MT\gamma_T
\]
Finally we can bound the cumulative regret by,
\begin{align*}
R_T = \sum_{t=1}^T r_t \leq \frac{\pi^2}{6} + 
2\beta_T\sum_{t=1}^T \sum_{j=1}^M \gpstdii{j}_{t}(\xpttii{j}) 
\leq \frac{\pi^2}{6} + \sqrt{8C_1\beta_T M T \gamma_T}
\end{align*}
\end{proof}


\subsection{Bounding the Information Gain $\gamma_T$}
\label{sec:appAnalysisInfGain}

For this we will use the following two results 
from \cite{srinivas10gpbandits}. \\

\begin{lemma}(Information Gain in GP, \cite{srinivas10gpbandits} Lemma5.3)
Using the basic properties of a GP, they show that 
\[
I(y_A; \func_A) = \frac{1}{2} \sum_{t=1}^{n} \log(1 + \eta^{-2}
  \sigma^2_{t-1}(x_t) )
\]
where $\sigma^2_{t-1}$ is the posterior variance after observing the first $t-1$
points. \\[\thmparaspacing]
\end{lemma}


\begin{theorem}(Bound on Information Gain, \cite{srinivas10gpbandits} Theorem 8)
Suppose that $\Xcal$ is compact and $\kernel$ is a kernel on $d$ dimensions
 satisifying Assumption~\ref{asm:partialDerivLipschitz}.
Let $n_T = C_9 T^\tau \log T$ where $C_9 = 4d+2$.
For any $T_* \in \{1, \dots, \min(T, n_T)\}$,
 let $B_\kernel(T_*) = \sum_{s>T_*}
\lambda_s$. Here $(\lambda_n)_{n\in \NN}$ are the eigenvalues of $\kernel$ w.r.t
the uniform distribution over $\Xcal$. 
Then,
\begin{equation*}
\gamma_T \leq  \inf_\tau  \left(
  \frac{1/2}{1-e^{-1}} \max_{r\in\cbr{1,\dots,T}} \left( T_* \log(r n_T/
\eta^2) + C_9 \eta^2 (1 - r/T) (T^{\tau+1} B_\kernel(T_*) + 1) \log T \right)
  + \bigO(T^{1-\tau /d}) 
\right)
\end{equation*}
\label{thm:srinivas}
\end{theorem}


\subsubsection{ \textbf{Proof of Theorem~\ref{thm:infGainBounds}-1}}
% \begin{proof}(\textbf{Proof of Theorem~\ref{thm:infGainBounds}-1})
\begin{proof}
We will use some bounds on the eigenvalues for the simple squared exponential
kernel given in \cite{seeger08information}. It was shown that the eigenvalues
$\{\lambdaii{i}_s\}$ of $\kernelii{i}$ satisfied $\lambdaii{i}_s \leq
c^dB^{s^{1/d_i}}$ where $B < 1$ (See Remark~\ref{rmk:eigvaldistros}).
Since the kernel is additive, and $\xii{i} \cap
\xii{j} = \emptyset$ the eigenfunctions corresponding to $\kernelii{i}$ and
$\kernelii{j}$ will be orthogonal. Hence the eigenvalues of $\kernel$ will
just be the union of the eigenvalues of the individual kernels -- i.e. 
$\{\lambda_s\} = \bigcup_{j=1}^M \{\lambdaii{j}_s \}$.  
As $B<1$, $\lambdaii{i}_s \leq c^dB^{s^{1/d}}$. Let $\Thash = \floor{T_*/M}$ and
$\alpha = -\log B$.
Then,
\begin{align*}
B_\kernel(T_*) &= \sum_{s>T_*} \lambda_s \leq Mc \sum_{s>\Thash} B^{s^{1/d}} \\
  &\leq c^dM \left( B^{\Thash^{1/d}} + \int_{\Thash}^\infty \exp(-\alpha x ^{1/d})
            \right) \ud x \\
  &\leq c^dM \left( B^{\Thash^{1/d}} + d \alpha^{-d} \Gamma(d, \alpha \Thash^{1/d})
            \right) \\ 
  &\leq c^dMe^{-\alpha \Thash^{1/d}} 
  \left( 1 + d! d \alpha^{-d} (\alpha \Thash^{1/d})^{d-1} \right)
\end{align*}
The last step holds true whenever $\alpha \Thash^{1/d} \geq 1$.
Here in the second step we bound the series by an integral used in the Maclaurin
Cauchy Integral test. In the second step we used the substitution $y =
\alpha x^{1/d}$ to simplify the integral. Here $\Gamma(s,x) = \int_x^\infty
t^{s-1} e^{-t} \ud t$ is the (upper) incomplete Gamma function. In the last step
we have used the following identity and the bound for integral $s$ and $x\geq 1$
\[
\Gamma(s,x) = (s-1)! e^{-x} \sum_{k=0}^{s-1} \frac{x^k}{k!} \leq s! e^{-x} x^{d-1}
\]
By using $\tau = d$ and by using
$T_* \leq (M+1) \Thash$, we
use Theorem~\ref{thm:srinivas} to obtain the following bound on $\gamma_T$,
\begin{align*}
\gamma_T &\leq 
  \frac{1/2}{1-e^{-1}} \max_{r\in\cbr{1,\dots,T}} \bigg( (M+1) \Thash \log(r n_T/
\eta^2) + \\
 &\hspace{0.2in} 
  C_9 \eta^2 (1 - r/T)  \log T \left( 1 + c^dMe^{-\alpha \Thash^{1/d}} T^{d+1} 
  \left( 1 + d! d \alpha^{-d} (\alpha \Thash^{1/d})^{d-1} \right)
  \right) \bigg)
\label{eqn:gammarbound} \numberthis
\end{align*}
Now we need to pick $\Thash$ so as to balance these two terms. We will choose
$\Thash = \left(\frac{\log(Tn_T)}{\alpha}\right)^d $ which is less than $\min(T,
n_T)/M$ for sufficiently large $T$. 
Then $e^{-\alpha \Thash^{1/d}} = 1/Tn_T$. Then the first term $S_1$ inside the
paranthesis is,
\begin{align*}
S_1 = (M+1) \log^d\left(\frac{Tn_T}{\alpha}\right)
        \log\left(\frac{rn_T}{\eta^2}\right) 
  &\in \bigO\left(M \left(\log(Tn_T)\right)^{d}\log(rn_T) \right) \\
  &\in \bigO\left(M \left(\log(T^{d+1}\log T)\right)^{d} \log(rT^d \log T)\right) \\
  &\in \bigO\left(M d^{d+1} (\log T)^{d+1} + M d^d (\log T)^d\log(r) \right)
\end{align*}
Note that the constant in front has exponential dependence on $d$ but we ignore
it since we already have $d^d$, $(\log T)^d$ terms.
The second term $S_2$ becomes,
\begin{align*}
S_2 &= 
  C_9 \eta^2 (1 - r/T)  \log T \left( 1 + \frac{c^dM}{Tn_T} T^{d+1} 
  \left( 1 + d! d \alpha^{-d} (\log(Tn_T)^{d-1} \right) 
  \right) \bigg) \\
  &\leq C_9 \eta^2 (1 - r/T)  \left( \log T  + \frac{c^dM}{C_9}  
  \left( 1 + d! d \alpha^{-d} (\log(Tn_T)^{d-1} \right) 
  \right) \bigg) \\
  &\leq C_9 \eta^2 (1 - r/T)  \left( \bigO(\log T) + \bigO(1) +
   \bigO(d! d^{d} (\log T)^{d-1}) \right) \bigg) \\
  &\in \bigO\left( (1-r/T)d! d^{d} (\log T)^{d-1} \right)
\end{align*}
Since $S_1$ dominates $S_2$, we should choose $r=T$ to maximize the RHS
in~\eqref{eqn:gammarbound}. This gives us,
\[
\gamma_T 
\;\in\; \bigO\left(M d^{d+1} (\log T)^{d+1}\right) 
\;\in\; \bigO\left(D d^{d} (\log T)^{d+1} \right) 
\]
\end{proof}



\subsubsection{ \textbf{Proof of Theorem~\ref{thm:infGainBounds}-2}}
% \begin{proof}(Proof of Theorem~\ref{thm:infGainBounds}-2)
\begin{proof}
Once again, we use bounds given in \cite{seeger08information}. 
It was shown that the eigenvalues $\{\lambdaii{i}_s\}$ for $\kernelii{i}$
satisfied $\lambdaii{i}_s \leq c^ds^{-\frac{2\nu+d_j}{d_j}}$
(See Remark~\ref{rmk:eigvaldistros}). By following a
similar argument to above we have 
$\{\lambda_s\} = \bigcup_{j=1}^M \{\lambdaii{j}_s \}$ and
$\lambdaii{i}_s \leq c^ds^{-\frac{2\nu+d}{d}}$. Let $\Thash = \floor{T_*/M}$.
Then,
\begin{align*}
B_\kernel(T_*) = \sum_{s>T_*} \lambda_s 
  \leq Mc^d\sum_{s>\Thash} s^{-\frac{2\nu+d}{d}} 
  \leq Mc^d\left( \Thash^{-\frac{2\nu+d}{d}} + 
      \int_{\Thash}^\infty s^{-\frac{2\nu+d}{d}}\right) 
  \leq C_8 2^d M\Thash^{1-\frac{2\nu+d}{d}}
%   \in \bigO\left(M\Thash^{1-\frac{2\nu+d}{d}} \right)
\end{align*}
where $C_8$ is an appropriate constant.
We set $\Thash = (Tn_T)^{\frac{d}{2\nu+d}} (\log(Tn_T))^{-\frac{d}{2\nu+d}}$ and
accordingly we have the following bound on $\gamma_T$ as a function of $\Thash \in
\{1,\dots, \min(T, n_T)/M\}$,
\begin{align*}
\gamma_T \leq 
  \inf_\tau \Bigg(
  \frac{1/2}{1-e^{-1}} \max_{r\in\cbr{1,\dots,T}} \bigg( (M+1) \Thash \log(r n_T/
\eta^2) +  
  C_9 \eta^2 (1 - r/T)   \left( \log T + C_8 2^d M \Thash \log(Tn_T) \right)
  \bigg) + \bigO(T^{1-\tau/d}) \Bigg)
\label{eqn:gammarboundmatern} \numberthis
\end{align*}
Since this is a concave function on $r$ we can find the optimum by setting the
derivative w.r.t $r$ to be zero. We get $r \in \bigO(T/2^d\log(Tn_T))$ and hence,
\begin{align*}
\gamma_T &\in \inf_\tau 
\left( \bigO\left( M \Thash \log\left(\frac{Tn_T}{2^d\log(Tn_T)}\right) \right)
  + \bigO\left(M 2^d \Thash \log(Tn_T) \right)
      + \bigO(T^{1-\tau/d}) \right) \\
&\in \inf_\tau \left(\bigO \left(M 2^d \log(Tn_T)
   \left(\frac{T^{\tau+1}\log(T)}{(\tau+1)\log(T) + \log\log T}\right)^\frac{d}{2\nu+d}
   \right) 
  + \bigO(T^{1-\tau/d}) \right) \\
&\in \inf_\tau \left(\bigO \left(M2^d\log(Tn_T)
   T^{\frac{(\tau+1)d}{2\nu+d}} \right) 
  + \bigO(T^{1-\tau/d}) \right) \\
&\in \bigO\left( M 2^d T^{\frac{d(d+1)}{2\nu + d(d+1)}} \log(T) \right)
\end{align*}
Here in the second step we have substitued the values for $\Thash$ first and
then $n_T$. In the last step we have balanced the polynomial dependence on $T$
in both terms by setting $\tau = \frac{2\nu d}{2\nu + d(d+1)}$. \\
\end{proof}

\begin{remark}
The eigenvalues and eigenfunctions for the kernel are defined with respect to a
base distribution on $\Xcal$. In the development of Theorem~\ref{thm:srinivas},
\cite{srinivas10gpbandits} draw $n_T$ samples from the uniform distribution on
$\Xcal$. Hence, the eigenvalues/eigenfunctions should be w.r.t the uniform
distribution. The bounds given in \cite{seeger08information} are for the uniform
distribution for the \matern kernel and a Gaussian Distribution for the Squared
Exponential Kernel. For the latter case, \cite{srinivas10gpbandits} argue that
the uniform distribution still satisfies the required tail constraints and
therefore the bounds would only differ up to constants.
\label{rmk:eigvaldistros}
\end{remark}


==> summaryTable.tex <==

\begin{table*}
\centering
\begin{tabular}{|l|c|c|}
\hline
Kernel & Squared Exponential & \matern \\
\hline
\rule{0pt}{3ex}
\gpbalgo on $D$\superscript{th} order Kernel  & $\sqrt{ D^{D+2} T (\log T)^{D+2}}$ &
  $\sqrt{D} 2^D T^{\frac{\nu + D(D+1)}{2\nu + D(D+1)}} \log T$ \\
\hline 
% \rule{0pt}{3ex}
% \gpbalgo on Additive Kernel & $\sqrt{ D T d^{d+1} (\log T)^{d+2}}$ & 
%   $\sqrt{Dd} 2^d T^{\frac{\nu + d(d+1)}{2\nu + d(d+1)}} \log T$ \\
% \hline 
\rule{0pt}{3ex}
\addgpbalgo on Additive Kernel & $\sqrt{ D^2 T d^{d} (\log T)^{d+2}}$ & 
  $D 2^d T^{\frac{\nu + d(d+1)}{2\nu + d(d+1)}} \log T$ \\
\hline
\end{tabular}
\label{tb:theorySummary}
\caption{Comparison of Cumulative Regret for \gpbalgo and \addgpbalgo for the
SE and \matern kernels.
}
\end{table*}


==> toyResults.tex <==

\begin{figure*}
\centering
\subfigure[]{
  \includegraphics[width=\imarrwthree]{images/SRD10d3} \hspace{\imhspthree}
  \vspace{\imlabelspace}
  \label{fig:SRD10d3}
}
\subfigure[]{
  \includegraphics[width=\imarrwthree]{images/SRD24d11} \hspace{\imhspthree}
  \vspace{\imlabelspace}
  \label{fig:SRD24d11}
}
\subfigure[]{
  \includegraphics[width=\imarrwthree]{images/SRD40d18}
  \vspace{\imlabelspace}
  \label{fig:SRD40d18}
} \\

\vspace{\imrowspace}
\subfigure[]{
  \includegraphics[width=\imarrwthree]{images/CRD10d3} \hspace{\imhspthree}
  \label{fig:CRD10d3}
}
\subfigure[]{
  \includegraphics[width=\imarrwthree]{images/CRD24d11} \hspace{\imhspthree}
  \label{fig:CRD24d11}
}
\subfigure[]{
  \includegraphics[width=\imarrwthree]{images/CRD40d18}
  \label{fig:CRD40d18}
} \\
\vspace{\imrowspace}

\subfigure[]{
  \includegraphics[width=\imarrwthree]{images/SRD40d5} \hspace{\imhspthree}
  \vspace{\imlabelspace}
  \label{fig:SRD40d5}
}
\subfigure[]{
  \includegraphics[width=\imarrwthree]{images/SRD96d5} \hspace{\imhspthree}
  \vspace{\imlabelspace}
  \label{fig:SRD96d5}
}
\subfigure[]{
  \includegraphics[width=\imarrwthree]{images/SRD40d18}
  \vspace{\imlabelspace}
  \label{fig:SRD41d18}
} \\

\vspace{\imrowspace}
\subfigure[]{
  \includegraphics[width=\imarrwthree]{images/CRD40d5} \hspace{\imhspthree}
  \label{fig:CRD40d5}
}
\subfigure[]{
  \includegraphics[width=\imarrwthree]{images/CRD96d5} \hspace{\imhspthree}
  \label{fig:CRD96d5}
}
\subfigure[]{
  \includegraphics[width=\imarrwthree]{images/CRD40d18}
  \label{fig:CRD41d5}
} \\
\caption[]{ \small
Results on the synthetic datasets. In all images the $x$-axis is the number
of queries and the $y$-axis is the regret in $\log$ scale. 
The first is $S_T$ for additive
functions with $(D,d,M)$ settings set to 
$(10,3,3)$, $(24,11,2)$, $(40,18,2)$ respectively. The second row is $R_T/T$ for
the same experiments. The third and fourth rows show similar curves for
the settings $(40,5,8)$, $(96,5,19)$ and $(144,42,4)$.
In some figures, the error bars are not visible since they are small and hidden
by the bullets. Here in \addgpbexpk we created as many groups as possible by
while ensuring the group size did not exceed $k$. For instance in
Fig~\subref{fig:SRD96d5} the green curve was run with $24$ groups each of size
$4$. \addgpbexps refers to a run of \addgpbalgo which knew the decomposition.
All figures were produced  by averaging over $20$ runs.
}
\label{fig:toy}
\vspace{\imtextspace}
\end{figure*}

